Towards Task-Specific Modular Gripper Fingers: Automatic Production of Fingertip Mechanics

The number of sequential tasks a single gripper can perform is significantly limited by its design. In many cases, changing the gripper fingers is required to successfully conduct multiple consecutive tasks. For this reason, several robotic tool change systems have been introduced that allow an automatic changing of the entire end-effector. However, many situations require only the modification or the change of the fingertip, making the exchange of the entire gripper uneconomic. In this paper, we introduce a paradigm for automatic task-specific fingertip production. The setup used in the proposed framework consists of a production and task execution unit, containing a robotic manipulator, and two 3D printers - autonomously producing the gripper fingers. It also consists of a second manipulator that uses a quick-exchange mechanism to pick up the printed fingertips and evaluates gripping performance. The setup is experimentally validated by conducting automatic production of three different fingertips and executing graspstability tests as well as multiple pick- and insertion tasks, with and without position offsets - using these fingertips. The proposed paradigm, indeed, goes beyond fingertip production and serves as a foundation for a fully automatic fingertip design, production and application pipeline - potentially improving manufacturing flexibility and representing a new production paradigm: tactile 3D manufacturing.

==> Text/_Discussion.tex <==
\section{Discussion}
% Finger Production
The experimental results show that our approach successfully provides a critical level of finger production and usage automation. The provided 3D printing pipeline potentially reduces the iteration time of gripper fingers significantly, since many manual steps have been automated and the standardized finger-bases reduces the required printing time. Decoupling the finger-base from the fingertip reduces further the design complexity, since only the fingertip geometry must be considered. 
% Quick-Exchange-Mechanism
Further, the presented quick-finger-exchange system increases operation flexibility of robot-arms, since multiple - for a certain operation specialized fingers - can be exchanged during the task-execution. The implementation of a finger-exchange system compared to an end-effector change approach, enables the continues usage of existing and potentially expensive gripper systems. This simplifies scaling the number of changeable "tools" from an economical as well as design point of view significantly. 
% Collective Manufacturing
Accordingly, the described setup can be used to quickly share, produce and apply fingertip design solutions developed at different fabrication locations. The collective learning approach [cit Lars], enables the common generation of skill knowledge, based on a collective of robot manipulators. Each robot learns a task by conducting different execution strategies. The results of this executions are shared with all other robots during the learning process. Similar to this shared learning approach, fingertips developed and iterated at different manufacturing facilities can be shared, produced and applied instantaneously. This potentially scales the number of fingertips and corresponding task applications a single robot-arm can conduct, significantly. The automatic production and quick-finger-exchange approach further supports this task-execution scaling. Different fingertips can be produced on the fly and changed during an application process. Accordingly, the number of tasks one robot can conduct is multiplied, since the fingers of different sub-tasks can be combined or stringed together. 

% Automatic Design Pipeline
Further, the presented approach can be considered as a base-line for a fully automatic finger design pipeline. The pipeline could automatically design, produce and apply finger-pairs for a given set of manipulation object and task scenarios. 

% Combine collective learning and manufacturing?
Such a fully automated and distributed manufacturing pipeline could potentially be combined with the described collective learning approach, to further increase task adaption automation, flexibility and efficiency. Here, the automatic finger production pipeline provides finger for many potentially distributed manufacturing cells, which learn the task-execution collectively together - based on the automatically generated and shared finger-design.
% --> transition to conclusion/future work

% Future work
Accordingly, future work will focus on the automatic fingertip generation aspect and the combination with collective task learning. Further, the development, selection and application of different finger-bases form-factors could potentially increase the application spectrum and flexibility. The current version of the finger-base is limited to a certain group of rather small and manipulation objects, which can only be grasped at the outer surface. 
